solc-verify: A Modular Verifier for Solidity Smart Contracts

We present solc-verify, a source-level verification tool for Ethereum smart contracts. Solc-verify takes smart contracts written in Solidity and discharges verification conditions using modular program analysis and SMT solvers. Built on top of the Solidity compiler, solc-verify reasons at the level of the contract source code, as opposed to the more common approaches that operate at the level of Ethereum bytecode. This enables solc-verify to effectively reason about high-level contract properties while modeling low-level language semantics precisely. The contract properties, such as contract invariants, loop invariants, and function pre- and post-conditions, can be provided as annotations in the code by the developer. This enables automated, yet user-friendly formal verification for smart contracts. We demonstrate solc-verify by examining real-world examples where our tool can effectively find bugs and prove correctness of non-trivial properties with minimal user effort.

==> ex_boogie_simple.tex <==
% !TEX root = paper.tex
% !TEX program = pdflatex

\begin{figure}[htb]
\begin{lstlisting}[language=Boogie]
var x : int;
var y : int;

procedure add(n : int)
	requires n >= 0;
	requires x == y;
	ensures  x == y;
{
	x := x + n;
	while (y < x)
		invariant y <= x;
	{
		y := y + 1;
	}
}
\end{lstlisting}
\caption{A simple Boogie program illustrating a procedure specified
with annotations.}
\label{fig:boogieexample}
\end{figure}


==> ex_solidity_simple.tex <==
% !TEX root = paper.tex
% !TEX program = pdflatex

\begin{figure}[htb]
\begin{lstlisting}[language=Solidity,escapechar=|]
/** @notice invariant x == y */ |\label{solidity::contract_inv}|
contract C {
  int x;
  int y;

  /** @notice precondition x == y
      @notice postcondition x == (y + n) */
  function add_to_x(int n) internal { |\label{solidity::annotated_internal}|
    x = x + n;
    require(x >= y); |\label{solidity::overflow_check}|
  }

  function add(int n) public {
    require(n >= 0);
    add_to_x(n);
    /** @notice invariant y <= x */ |\label{solidity::loop_invariant}|
    while (y < x) {
      y = y + 1;
    }
  }
}
\end{lstlisting}
%
\caption{A simple annotated Solidity example. The contract
maintains that $x$ and $y$ are always equal. The check
at line \ref{solidity::overflow_check} ensures that overflow
cannot happen.}
%
\label{fig:solidityexample}
\end{figure}

